PointOBB-v2: Towards Simpler, Faster, and Stronger Single Point Supervised Oriented Object Detection

Single point supervised oriented object detection has gained attention and made initial progress within the community. Diverse from those approaches relying on one-shot samples or powerful pretrained models (e.g. SAM), PointOBB has shown promise due to its prior-free feature. In this paper, we propose PointOBB-v2, a simpler, faster, and stronger method to generate pseudo rotated boxes from points without relying on any other prior. Specifically, we first generate a Class Probability Map (CPM) by training the network with non-uniform positive and negative sampling. We show that the CPM is able to learn the approximate object regions and their contours. Then, Principal Component Analysis (PCA) is applied to accurately estimate the orientation and the boundary of objects. By further incorporating a separation mechanism, we resolve the confusion caused by the overlapping on the CPM, enabling its operation in high-density scenarios. Extensive comparisons demonstrate that our method achieves a training speed 15.58x faster and an accuracy improvement of 11.60%/25.15%/21.19% on the DOTA-v1.0/v1.5/v2.0 datasets compared to the previous state-of-the-art, PointOBB. This significantly advances the cutting edge of single point supervised oriented detection in the modular track.

==> Tables/t4_label_assignment.tex <==
\begin{table}[H]
\centering
\caption{Ablation study of different label assignment strategies.}
\vspace{2mm}
\begin{tabular}{ccc|c}
\toprule
\textbf{Assign 2}     & \textbf{Assign 1}     & \textbf{Assign 3}     & \textbf{mAP}$_\text{50}$ \\ \hline
$\checkmark$ &              &              & \\
$\checkmark$ & $\checkmark$ &              &     \\
$\checkmark$ &              & $\checkmark$ &     \\
$\checkmark$ & $\checkmark$ & $\checkmark$ &     \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/t5_PCA_sample_method.tex <==
\begin{table}[!tb]
  \centering
  \begin{minipage}{0.45\textwidth}  % Left side with two tables
    \centering
    % First table on the left
    \caption{Ablation study of sample methods.}
    \label{tab:sample_method}
    % \vspace{1.5mm}
    % \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
    \textbf{Sample}  & Probabilistic & Weighted \\ \hline
    \textbf{mAP}$_\text{50}$ & 41.40 & \textbf{44.85} \\ \bottomrule
    \end{tabular}
    % Second table on the left
    \vspace{4mm}
    % \caption{Ablation study of PCA Size.}
    % % \vspace{1.5mm}
    % \resizebox{0.98\textwidth}{!}{
    % \begin{tabular}{c|cccc}
    % \toprule
    % \textbf{PCA Size} & 5 & 7 & 9 & 11 \\ \hline
    % \textbf{mAP}$_\text{50}$ & 43.35 & \textbf{44.85} & 44.17 & 43.63 \\ \bottomrule
    % % \caption{Ablation study of dense object processing modules.}
    % % % \vspace{1.5mm}
    % % \begin{tabular}{c|c}
    % % \toprule
    % %  Vector Constrain & \textbf{mAP}$_\text{50}$                  \\ \hline
    % %                   & 27.88 \\
    % %  $\checkmark$     & \textbf{44.85} \\ \bottomrule
    % \end{tabular}}
    \caption{Ablation study of dense object processing modules.} %"w" and "w/o" indicate the "with" and "without" of the module, respectively.}
    \label{tab:vector_constrain}
    \begin{tabular}{c|cc}
    \toprule
     Vector Constraint         & w/o     & w                 \\ \hline
     \textbf{mAP}$_\text{50}$ & 27.88 & \textbf{44.85}             \\ \bottomrule
    \end{tabular}
  \end{minipage}%
  \quad
  % \hspace{0.05\textwidth}  % Adjust the horizontal space between left and right
  \begin{minipage}{0.50\textwidth}  % Right side with one table
    \centering
    % Table on the right
    \caption{Ablation study of PCA Size.}
    \label{tab:pca_size}
    % \vspace{1.5mm}
    % \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cc}
    \toprule
    \textbf{PCA Size} & \textbf{mAP}$_\text{50}$ \\
    \midrule
    5 & 43.35\\
    7 & \textbf{44.85}\\
    9 & 44.17\\
    11 & 43.63\\ \bottomrule
    
    % \caption{Ablation study of dense object processing modules.}
    % % \vspace{1.5mm}
    % \begin{tabular}{c|c}
    % \toprule
    %  Vector Constrain & \textbf{mAP}$_\text{50}$                  \\ \hline
    %                   & 27.88 \\
    %  $\checkmark$     & \textbf{44.85} \\ \bottomrule
    \end{tabular}
  \end{minipage}
\end{table}


==> Tables/t5t6t7t8_2r2c.tex <==
\begin{table}[!tb]
  \centering
  \begin{minipage}{0.45\textwidth}  % Left side with two tables
    \centering
    % First table on the left
    \caption{Ablation study of sample methods.}
    \label{tab:sample_method}
    % \vspace{1.5mm}
    % \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
    \textbf{Sample}  & Probabilistic & Weighted \\ \hline
    \textbf{mAP}$_\text{50}$ & 41.40 & \textbf{44.85} \\ \bottomrule
    \end{tabular}
    % Second table on the left
    \vspace{4mm}
    % \caption{Ablation study of PCA Size.}
    % % \vspace{1.5mm}
    % \resizebox{0.98\textwidth}{!}{
    % \begin{tabular}{c|cccc}
    % \toprule
    % \textbf{PCA Size} & 5 & 7 & 9 & 11 \\ \hline
    % \textbf{mAP}$_\text{50}$ & 43.35 & \textbf{44.85} & 44.17 & 43.63 \\ \bottomrule
    % % \caption{Ablation study of dense object processing modules.}
    % % % \vspace{1.5mm}
    % % \begin{tabular}{c|c}
    % % \toprule
    % %  Vector Constrain & \textbf{mAP}$_\text{50}$                  \\ \hline
    % %                   & 27.88 \\
    % %  $\checkmark$     & \textbf{44.85} \\ \bottomrule
    % \end{tabular}}
    \caption{Ablation study of dense object processing modules.} %"w" and "w/o" indicate the "with" and "without" of the module, respectively.}
    \label{tab:vector_constrain}
    \begin{tabular}{c|cc}
    \toprule
     Vector Constraint         & w/o     & w                 \\ \hline
     \textbf{mAP}$_\text{50}$ & 27.88 & \textbf{44.85}             \\ \bottomrule
    \end{tabular}
  \end{minipage}%
  \quad
  % \hspace{0.05\textwidth}  % Adjust the horizontal space between left and right
  \begin{minipage}{0.50\textwidth}  % Right side with one table
    \centering
    % Table on the right
    % \caption{Ablation study of PCA Size.}
    % \label{tab:pca_size}
    % % \vspace{1.5mm}
    % % \resizebox{0.98\textwidth}{!}{
    % \begin{tabular}{cc}
    % \toprule
    % \textbf{PCA Size} & \textbf{mAP}$_\text{50}$ \\
    % \midrule
    % 5 & 43.35\\
    % 7 & \textbf{44.85}\\
    % 9 & 44.17\\
    % 11 & 43.63\\ \bottomrule
    \caption{Ablation study of PCA Size.}
    % \vspace{1.5mm}
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{PCA Size} & 5 & 7 & 9 & 11 \\ \hline
    \textbf{mAP}$_\text{50}$ & 43.35 & \textbf{44.85} & 44.17 & 43.63 \\ \bottomrule
    
    % \caption{Ablation study of dense object processing modules.}
    % % \vspace{1.5mm}
    % \begin{tabular}{c|c}
    % \toprule
    %  Vector Constrain & \textbf{mAP}$_\text{50}$                  \\ \hline
    %                   & 27.88 \\
    %  $\checkmark$     & \textbf{44.85} \\ \bottomrule
    \end{tabular}
  \end{minipage}
\end{table}


==> Tables/t6_PCA_size.tex <==
\begin{table}[H]
\centering
\caption{Ablation study on the effect of sample length (PCA size) on \textbf{mAP$_\text{50}$}}
\vspace{1.5mm}
\begin{tabular}{c|c}
\toprule
\textbf{PCA Size} & \textbf{mAP}$_\text{50}$ \\ \hline
5        & 43.52 \\
7        & \textbf{43.82} \\
9        & 43.51 \\
11       & 43.65 \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/t7_dense_processing.tex <==
\begin{table}[H]
\centering
\caption{Ablation study of two dense object processing modules.}
\vspace{1.5mm}
\begin{tabular}{cc|c}
\toprule
Center Factor & Vector Constrain & \textbf{mAP}$_\text{50}$                  \\ \hline
              &                  &  \\
$\checkmark$  &                  &  \\
              & $\checkmark$     &  \\
$\checkmark$  &   $\checkmark$   &  \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/t8_random_shift_point.tex <==
\begin{table}[!tb]
\centering
\caption{Ablation of point annotations inaccuracy.}
\begin{tabular}{c|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Point Range}} & \multicolumn{2}{c|}{\textbf{DOTA-v1.0}} & \multicolumn{2}{c|}{\textbf{DOTA-v1.5}} & \multicolumn{2}{c}{\textbf{DOTA-v2.0}} \\ \cline{2-7} 
                             & \textbf{mIoU}           & \textbf{mAP}           & \textbf{mIoU}           & \textbf{mAP}           & \textbf{mIoU}           & \textbf{mAP}          \\ \hline
0\%                          & 45.40 & 44.85 & 43.65 & 36.39 & 42.91 & 27.22 \\
10\%                         & 42.89 & 42.30 & 41.85 & 34.20 & 41.46 &              \\
20\%                         & 40.22 & 38.46 & 39.47 & 30.95 & 39.30 &              \\ \bottomrule
\end{tabular}
\end{table}
